Parallelizing greedy for submodular set function maximization in matroids and beyond

We consider parallel, or low adaptivity, algorithms for submodular function maximization. This line of work was recently initiated by Balkanski and Singer and has already led to several interesting results on the cardinality constraint and explicit packing constraints. An important open problem is the classical setting of matroid constraint, which has been instrumental for developments in submodular function maximization. In this paper we develop a general strategy to parallelize the well-studied greedy algorithm and use it to obtain a randomized $\left(\frac{1}{2} - \epsilon\right)$-approximation in $\operatorname{O}\left( \frac{\log^2 n}{\epsilon^2} \right)$ rounds of adaptivity. We rely on this algorithm, and an elegant amplification approach due to Badanidiyuru and Vondr\'ak to obtain a fractional solution that yields a near-optimal randomized $\left( 1 - 1/e - \epsilon \right)$-approximation in $O\left( {\frac{\log^2 n}{\epsilon^3}} \right) $ rounds of adaptivity. For non-negative functions we obtain a $\left( {3-2\sqrt{2}}\right)$-approximation and a fractional solution that yields a $\left( {\frac{1}{e} - \epsilon}\right)$-approximation. Our approach for parallelizing greedy yields approximations for intersections of matroids and matchoids, and the approximation ratios are comparable to those known for sequential greedy.

==> overview.tex <==
\subsection{High-Level Overview}

\emph{This section will be deleted.}

Let us assume for concreteness the canonical problem of maximizing a
monotone submodular function subject to a matroid constraint, which
was our original motivating. We give an overview of our techniques and
algorithm in this particular setting and discuss generalizations
afterwards.

Let $\defmatroid$ be a matroid and $\defnnsubmodular$ a monotone
submodular function. The goal is to compute, in parallel, an
independent set $I \in \independents$ maximizing $f(I)$. It is
well-known, from the simple case of maximum coverage s.t.\ a
cardinality constraint in the sequential setting, that it is NP-Hard
to achieve better than an approximation ratio better than
$1 - e^{-1} \approx .63$. This approximation factor was first obtained
in the sequential setting by \citet{ccpv} (up to an
$\epsless$-multiplicative factor, for any fixed $\eps$).

Consider the simple greedy algorithm for this optimization problem,
given in \reffigure{greedy}. The greedy algorithm starts with an empty set
$S = \emptyset$, and greedily adds to $S$ the element $e$ maximizing
$f(S + e)$ subject to $S + e \in \independents$. It terminates when
there are no longer any elements that can be added to $S$.
\begin{figure}
  \begin{algorithm}{greedy}{$\defmatroid$,$\defnnsubmodular$}
  \item $S \gets \emptyset$
  \item while $S$ is not a base
    \begin{steps}
    \item $e \gets \argmax[d]{f_S(d) \where I + d \in \independents}$
    \item $S \gets S + e$
    \end{steps}
  \item return $S$
  \end{algorithm}
  \caption{A greedy $2$-approximation for maximizing a monotone
    submodular function subject to a matroid
    constraint.\labelfigure{greedy}}
\end{figure}
The greedy algorithm has an approximation ratio of $1/2$, short of the
optimal $(1-e^{-1})$-approximation schemes. This suboptimal ratio is
not the primary concern because \textit{a priori} it is not clear how
to get any constant factor approximation for matroids in
parallel. (Moreover, a $1/2$ approximation ratio can be amplified to
$1-e^{-1}$; more on this later.)  The greater problem in our setting
is that it is inherently very sequential. The number of iterations,
$\rank{\matroid}$, can be as large as $n$. One hopes to ``flatten''
the iterations, but each chosen element $e$ depends on the previously
selected elements $S$ at 2 critical points: (a) the marginal value
$f_S(e)$ decreases as $S$ increases due to submodularity, and (b) we
cannot take $e$ if $S + e$ is infeasible.

\subsubsection{Randomized greedy blocks}

It is clear that to obtain $\poly{\log n, \reps}$ depth, we cannot
take just one element at a time, and would prefer to somehow take,
say, $\rank{\matroid} / \poly{\log n, \reps}$ elements in each
parallel round. In fact, we do not even take a set per iteration, but
pairs of sets that we call ``greedy blocks''.

For any set system $\defmatroid$, a \defterm{$\epsless$-greedy block}
consists of a randomized pair of sets $(R,S)$ s.t.\
\begin{enumerate}
\item $R \subseteq S$ and $R \in \independents$.
\item
  \begin{math}
    \evof{f(R)} \geq \epsless \evof{\sizeof{S}} \parof{\max_{e} f(e)}.
  \end{math}
\end{enumerate}
We are interested in randomized greedy blocks not only w/r/t
$\matroid$ and $f$, but the contracted matroid $\matroid / Q$ and
marginal values $f_Q$ for various sets $Q \subseteq \groundset$.

Greedy blocks are general and implicit in many existing algorithms.
For example, the standard greedy algorithm can be seen as repeatedly
taking greedy blocks $(R,S)$ in the residual, where $R$ and $S$ are
the same singleton set containing the element with maximum marginal
value. Greedy blocks are designed to be relaxed but sufficient
conditions to carry through the standard greedy analysis.

Note that $S$ is not required to be independent, but we still require
an independent certificate $R \subseteq S$ that captures most of the
value of $S$.  At the end of the day, we will output a union of the
independent $R$-components of the greedy blocks which will form a
feasible solution. Allowing $S$ to be dependent is an important degree
of freedom that is used to make measurable progress.  The dependent
$S$-components are aggressively pushed until either (a) $S$ spans a
large fraction of $\matroid$, or (b) the residual values of $f_S$ are
substantially smaller than $f$ in some quantified sense.

\subsubsection{Greedy sampling}

\labelsection{overview:greedy-sample}

We generate greedy blocks for matroids by a ``greedy'' sampling
procedure.  We focus on the setting where all elements
$e \in \groundset$ have margin
$\epsless \lambda \leq f(e) \leq \lambda$ for some $\lambda >0$.  For
a carefully chosen value $\delta > 0$, we let $S$ sample each element
in the ground set uniformly at random. $S$ may be dependent. We then
prune any element in the set that is either (a) spanned by the other
sampled elements or (b) has marginal value less than $\eps\lambda$
w/r/t the other sampled elements. The pruning step leaves an
independent subset $R \subseteq S$ where each element contributes at
least $\epsless \lambda$ to $f(R)$.

The high-level algorithm is very simple, and its behavior depends on
the choice of $\delta$.  As $\delta$ increases, and $S$ grows with it,
submodularity pushes down the expected value of $S$ per sampled
element, and the expected span of $S$ increases. In turn, the
likelihood of pruning increases, and the ratio $f(R) / \sizeof{S}$
decreases in expectation. Conversely, as we take $\delta$ down to 0,
$R$ converges to $S$ in expectation, and for sufficiently small
$\delta$, $(R,S)$ is a greedy block. We define the ``sufficiently
small'' threshold to be such that in expectation, (a) at least
$\epsless$-fraction of $\groundset$ has marginal value
$\geq \epsless \lambda$ w/r/t $S$, and (b) at least
$\epsless$-fraction of $\groundset$ is not spanned by $S$. Any
$\delta$ satisfying both (a) and (b), it is shown, produces a greedy
block $(R,S)$.

We greedily maximize $\delta$ s.t.\ the above constraints for the sake
of efficiency. Maximality ensures we reach the breaking point of one
of the two limiting conditions. If condition (a) is tight, when many
of the elements have their marginal value drop below
$\epsless \lambda$. If $\delta$ is large enough that (b) is tight,
then a large fraction of $\groundset$ should be sampled by $S$.
sample spans about an $\eps$-fraction of the entire matroid. Either
way, we expect to substantially decrease the number of un-spanned
elements with marginal value $\geq \epsless \lambda$.

We prove the following in greater generality in
\refsection{greedy-sample}.
\begin{namedtheorem*}{\reftheorem{greedy-sample} (for matroids)}
  \thegmstheorem[matroid]
\end{namedtheorem*}

\subsubsection{Iteration by greedy blocks}

We now iterate along greedy blocks, where each iteration is w/r/t the
residual of previously selected greedy blocks.  We start with empty
sets $R,S = \emptyset$. We repeatedly generate $\epsless$-greedy
blocks $(R',S')$ w/r/t the contracted matroid $\matroid / S$ and the
marginal values $f_S$, and then add $R'$ to $R$ and $S'$ to
$S$.

The upper bound $\lambda$ is chosen according to the standard
technique of thresholding, where we hold onto the same value of
$\lambda$ until $\epsless \lambda$ becomes an upper bound.  The
thresholding allows us to bound the depth. $\lambda$ can be decreased
a limited number of times before the marginal values of the remaining
elements are negligible. Within a fixed $\lambda$, due to part (ii) of
\reftheorem{greedy-sample}, we expect to call \algo{greedy-sample} a
limited number of times before the marginal values of the remaining
elements are less than $\epsless \lambda$.

In \refsection{greedy-blocks} we prove the following theorem (more
generally), which says that the iterative process of greedy blocks
essentially behaves like the sequential greedy algorithm.
\begin{namedtheorem*}{\reftheorem{block-greedy} (for monotone
    submodular functions in matroids)}
  Let $\defmatroid$ be a matroid and $\defnnsubmodular$ a monotone
  submodular function. With $\bigO{\frac{\log^2 n}{\eps^2}}$ calls to
  \algo{greedy-sample} in expectation, we can compute
  $I \in \independents$ such that
  \begin{center}
    \begin{math}
      \ef{I} \geq \epsless \ef{T}{I}
    \end{math}
    for all $T \in \independents$.
  \end{center}
\end{namedtheorem*}

Since $\ef{T}{I} \geq f(T) - \ef{I}$ for monotone $f$,
\reftheorem{block-greedy} implies that we can compute a
$\prac{1-\eps}{2}$-approximate independent set with polylogarithmic
adaptivity.

\subsubsection{Multilinear amplification}

Iteration along greedy blocks produces independent sets that match the
greedy algorithm in performance (in expectation and with
$\epsless$-multiplicative loss). This gives a near-2 approximation,
short of the desired near-$\parof{1 - 1/e}$ approximation factor for
the sequential setting.  \citet{bv} showed how to amplify a near-2
approximation into a near-$\parof{1 - 1/e}$ approximate fractional
solution, as a convex combination of $\bigO{\reps}$ near-2
approximations w/r/t submodular functions induced by the multilinear
relaxation. We call this process ``multilinear amplification''.

\begin{namedtheorem*}{\reftheorem{multilinear-amplification} (applied
    to matroids)}
  Let $\defmatroid$ be a matroid, and let $\defnnsubmodular$ be a
  monotone submodular function. Suppose one has access to an oracle
  that, given a submodular function $g$, returns a (possible
  randomized) set
  \begin{center}
    \begin{math}
      I \in \independents
    \end{math}
    such that
    \begin{math}
      \evof{g(I)} \geq \epsless \evof{g_I(T)}.
    \end{math}
  \end{center}
  With $\bigO{\reps}$ calls to this oracle, one can compute a convex
  combination of $\bigO{\reps}$ independent sets $x \in
  \convex{\independents}$ such that
  \begin{align*}
    \mlf{x} \geq \epsless \parof{1 - e^{-1}} \opt,
  \end{align*}
  where $\mlf$ is the multilinear extension of $f$, and
  $\opt = \max_{I \in \independents} f(I)$.
\end{namedtheorem*}

In the sequential setting, a fractional independent set can be rounded
to an integral independent set without loss (in expectation). Although
rounding in parallel is not known and remains an interesting open
question, applying \reftheorem{multilinear-amplification} to
\reftheorem{block-greedy} implies an near-optimal approximation to the
maximum value of any independent set with polylogarithmic depth.

\begin{corollary}
  Let $\defmatroid$ be a matroid and $\defnnsubmodular$ a monotone
  submodular function. With $\bigO{\log{n}/\eps^2}$ adaptivity, one
  can compute a convex combination $x$ of $\bigO{\reps}$ independent
  sets such that
  \begin{align*}
    \evof{F(x)} \geq \epsless \parof{1 - e^{-1}} \opt,
  \end{align*}
  where $\opt = \max_{I \in \independents} f(I)$. This implies a
  $\epsless (1-e^{-1})$-approximation to the value $\opt$ with
  $\bigO{\log{n}/\eps^2}$ depth.
\end{corollary}


\subsubsection{Parallel greedy algorithms in general}

We highlight monotone submodular function maximization in matroids
because they are an important test case in combinatorial
optimization. The overall framework is more general, and tries to show
that
\begin{center}
  \emph{the greedy algorithm for submodular maximization can be
    implemented in parallel}.
\end{center}
It is well-known that the sequential greedy algorithm gives or leads
to approximation algorithms for other combinatorial constraints and
generally nonnegative submodular functions. The same results extend
here.

Looking back, we first observe that the greedy sampling procedure
(\reftheorem{greedy-sample} in full generality) does not require
$\defmatroid$ to be a matroid, or $f$ to be monotone or even
nonnegative.  It is important to not assume nonnegativity because the
marginal functions $f_S$ that arise in the iterative framework are not
nonnegative.  \reftheorem{greedy-sample} extends to set systems with a
well-defined notion of ``span'' that is slightly weaker than the span
function in matroids, discussed in greater detail in
\refsection{matroid-combinations}. In particular,
\reftheorem{greedy-sample} extends to standard combinations of
matroids such as matroid intersections and matchoids.

The iterative analysis of greedy blocks, \reftheorem{greedy-blocks},
also does not require $f$ to be monotone or nonnegative. Moreover, the
proof is very similar to the sequential greedy analysis, generalized
for greedy blocks. It is well-known that the sequential greedy
analysis can be modified for other systems such as matroid
intersection. The same modifications can be made here as well.

Multilinear amplification is also very general. While \cite{bv}
focuses specifically on matroid constraint, it is not difficult to see
that it holds for any set system and varying approximation ratio
given by the oracle. Moreover, it is shown (in
\reftheorem{nn-multilinear-amplification}) that multilinear
amplification can be extended to general nonnegative submodular
functions. Nonnegative multilinear amplification is to
\algo{measured-greedy} what monotone multilinear amplification is to
\algo{continuous-greedy}.

All put together, the results extend to low-adaptivity approximation
for nonnegative submodular functions and more general combinations of
matroids, as follows.

\begin{corollary}
  Let $\defmatroid$ be a matroid and $\defnnsubmodular$ a nonnegative
  submodular function. With $\bigO{\log^2 (n) / \eps^3}$ adaptivity,
  one can obtain a $\epsless e^{-1}$-approximation to the maximum
  value of any independent set. A constant factor approximate
  independent set can be obtained in $\bigO{\log^2 (n) / \eps^2}$
  adaptivity.
\end{corollary}

\begin{corollary}
  Let $\defmatroid$ be a $k$-matchoid and $\defnnsubmodular$ a
  monotone submodular function. With $\bigO{\log^2(n) / \eps^2}$
  adaptivity, one can obtain a $\frac{1 - \eps}{k+1}$-approximate
  maximum value independent set. With $\bigO{\log^2(n) / \eps^3}$
  adaptivity, one can obtain a
  $\epsless \parof{1 - e^{-1/k}}$-approximation to the maximum value
  of any independent set.
\end{corollary}

In conclusion, the combination of a greedy block iteration scheme, a
low-depth sampling procedure for generating greedy blocks, and
multilinear amplification produces a low-depth approximation of the
sequential greedy algorithm. The framework closes the gap between the
parallel and sequential settings not only w/r/t obtaining competitive
bounds, but conceptually as well.

